Generalized Radio Environment Monitoring for Next Generation Wireless Networks

Enabling technologies of 5G and beyond wireless communication networks, such as millimeter-wave communication, beamforming, and multiple-input multiple-output (MIMO) antenna systems, are becoming increasingly dependent on accurate information of the physical environment for optimized communication performance. The acquisition of this information is a significant challenge, which can be eased by knowledge of the radio environment. Radio environment mapping (REM) has long been considered an enabler of cognitive radios (CRs). However, the limitations of radios effectively confined the application of REM to spectrum sensing and interference mapping. With the advent of more capable software-defined radios and advanced networks, the idea of a truly intelligent communication system empowered by enhanced REM can be realized. To this effect, we propose the generalized radio environment monitoring (G-REM) concept to include all aspects of the radio environment. We outline a general, self contained framework which enables radio environment monitoring in standalone devices. The presented G-REM framework comprises of different information sources, sensing methods, sensing modes, and mapping techniques to enable the realization of more reliable, secure, efficient, and faster future wireless networks. The accompanying challenges and future research direction are also provided.

==> AcronymList.tex <==
\usepackage{etoolbox}
\makeatletter
\newif\ifAC@uppercase@first%
\def\Aclp#1{\AC@uppercase@firsttrue\aclp{#1}\AC@uppercase@firstfalse}%
\def\AC@aclp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acl{#1}s%
	\fi%
}%
\def\Acp#1{\AC@uppercase@firsttrue\acp{#1}\AC@uppercase@firstfalse}%
\def\AC@acp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@ac{#1}s%
	\fi%
}%
\def\Acfp#1{\AC@uppercase@firsttrue\acfp{#1}\AC@uppercase@firstfalse}%
\def\AC@acfp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acf{#1}s%
	\fi%
}%
\def\Acsp#1{\AC@uppercase@firsttrue\acsp{#1}\AC@uppercase@firstfalse}%
\def\AC@acsp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acs{#1}s%
	\fi%
}%
\edef\AC@uppercase@write{\string\ifAC@uppercase@first\string\expandafter\string\MakeUppercase\string\fi\space}%
\def\AC@acrodef#1[#2]#3{%
	\@bsphack%
	\protected@write\@auxout{}{%
		\string\newacro{#1}[#2]{\AC@uppercase@write #3}%
	}\@esphack%
}%
\def\Acl#1{\AC@uppercase@firsttrue\acl{#1}\AC@uppercase@firstfalse}
\def\Acf#1{\AC@uppercase@firsttrue\acf{#1}\AC@uppercase@firstfalse}
\def\Ac#1{\AC@uppercase@firsttrue\ac{#1}\AC@uppercase@firstfalse}
\def\Acs#1{\AC@uppercase@firsttrue\acs{#1}\AC@uppercase@firstfalse}
\robustify\Aclp
\robustify\Acfp
\robustify\Acp
\robustify\Acsp
\robustify\Acl
\robustify\Acf
\robustify\Ac
\robustify\Acs
\makeatother
%% FOR REM MAGAZINE

\acrodef{IoT}[IoT]{internet of things}
\acrodef{BS}[BS]{base station}
\acrodef{REM}[REM]{radio environment map}
\acrodef{GREM}[G-REM]{generalized radio environment monitoring}
\acrodef{CR}[CR]{cognitive radio}
\acrodef{AP}[AP]{access point}
\acrodef{UE}[UE]{user equipment}
\acrodef{REA}[REA]{radio environment awareness}
\acrodef{RES}[RES]{radio environment sensing}
\acrodef{RSSI}[RSSI]{received signal strength indicator}
\acrodef{SNR}[SNR]{signal-to-noise ratio}
\acrodef{RES}[RES]{radio environment sensing}
\acrodef{WLAN}[WLAN]{wireless local area network}
\acrodef{V2X}[V2X]{vehicle-to-everything}
\acrodef{eMBB}[eMBB]{enhanced mobile broadband}
\acrodef{mMTC}[mMTC]{massive machine type communication}
\acrodef{uRLLC}[uRLLC]{ultra-reliable low latency communication}
\acrodef{CoMP}[CoMP]{coordinated multipoint}
\acrodef{LTE}[LTE]{Long Term Evolution}
\acrodef{RAN}[RAN]{radio access network}
\acrodef{SON}[SON]{self-organizing network}
\acrodef{MAC}[MAC]{medium access control}
\acrodef{PHY}[PHY]{physical layer}
\acrodef{5G}[5G]{fifth generation}
\acrodef{6G}[6G]{sixth generation}
\acrodef{WLAN}[WLAN]{wireless local area network}
\acrodef{radar}[radar]{radio detection and ranging}
\acrodef{JRC}[JRC]{joint radar and communication}
\acrodef{DFT}[DFT]{discrete Fourier transform}
\acrodef{UE}[UE]{user equipment}
\acrodef{LoS}[LoS]{line-of-sight}
\acrodef{NLoS}[NLOS]{non-line-of-sight}
\acrodef{ATSSS}[ATSSS]{access traffic steering switching and splitting}
\acrodef{CSI}[CSI]{channel state information}
\acrodef{OFDM}[OFDM]{orthogonal frequency division multiplexing}
\acrodef{D2D}[D2D]{device-to-device}
\acrodef{V2V}[V2V]{vehicle-to-vehicle}
\acrodef{QoS}[QoS]{quality of service}
\acrodef{MIMO}[MIMO]{multiple-input multiple-output}
\acrodef{mmWave}[mmWave]{millimeter-wave}
\acrodef{THz}[THz]{terahertz}
\acrodef{RIS}[RIS]{reconfigurable intelligent surface}
\acrodef{VLC}[VLC]{visible light communication}
\acrodef{RF}[RF]{radio frequency}
\acrodef{XR}[XR]{extended reality}
\acrodef{LDHMC}[LDHMC]{long-distance high mobility communication}
\acrodef{eLPC}[eLPC]{extremely low-power communication}
\acrodef{5QI}[5QI]{\ac{5G} \ac{QoS} identifier}
\acrodef{mMIMO}[mMIMO]{massive \ac{MIMO}}
\acrodef{SWIPT}[SWIPT]{simultaneous wireless information and power transfer}
\acrodef{BSA}[BSA]{blind signal analysis}
\acrodef{NOMA}[NOMA]{non-orthogonal multiple access}
\acrodef{CoMP}[CoMP]{coordinated multipoint}
\acrodef{TP}[TP]{transmission point}
\acrodef{TDD}[TDD]{time-division duplexing}
\acrodef{FDD}[FDD]{frequency-division duplexing}
